Online Dense Subgraph Discovery via Blurred-Graph Feedback

Dense subgraph discovery aims to find a dense component in edge-weighted graphs. This is a fundamental graph-mining task with a variety of applications and thus has received much attention recently. Although most existing methods assume that each individual edge weight is easily obtained, such an assumption is not necessarily valid in practice. In this paper, we introduce a novel learning problem for dense subgraph discovery in which a learner queries edge subsets rather than only single edges and observes a noisy sum of edge weights in a queried subset. For this problem, we first propose a polynomial-time algorithm that obtains a nearly-optimal solution with high probability. Moreover, to deal with large-sized graphs, we design a more scalable algorithm with a theoretical guarantee. Computational experiments using real-world graphs demonstrate the effectiveness of our algorithms.

==> sec/nesterov.tex <==
\section*{Nesterov's algorithm}


==> sec/supp_rev.tex <==
\begin{onecolumn}
%\twocolumn[
\icmltitle{Supplementary Material:\\
\vspace{2mm}
Online Dense Subgraph Discovery via Blurred-Graph Feedback}

\appendix

\input{sec/related.tex}
%\section{Related work on the densest subgraph problem}\label{sec:related}

% \section{Overview of multi-armed bandits and related work on best arm identification}\label{apx:related_bandit}
% In this section, we briefly describe the framework of the stochastic {\em multi-armed bandit} and related work on {\em best arm identification}.


% \subsection{Multi-armed bandits and its variants}
% The multi-armed bandit (MAB) is a sequential decision making model, in which at each time step, 
% a player takes an action and observes a stochastic reward as a response~\cite{Lai1985}.
% An action is usually called an {\em arm}, 
% which characterizes the decision making problem of a player in the following stochastic game. 
% Suppose that there are $m$ arms.
% At each round $t=1, 2, \ldots,$
% the player must choose an arm to play from $m$ arms.
% When each arm $i$ is pulled, the player can observe a stochastic reward sampled from an unknown probability distribution.
% The most well-studied objective is {\em regret minimization},i.e.,
% to minimize the cumulative regret or maximize the cumulative reward~\citep{ bubeck2012,cesa2006prediction}.
% Another popular objective is to identify the best arm i.e., the arm with the maximum expected reward among $m$ arms by interacting the game.
% This problem,
% called {\em  pure exploration} or {\em best arm identification} in the MAB,
% has received much attention recently~\citep{Audibert2010, Chen2015,Even2002,Even2006,Jamieson2014,kaufmann2016}.


% A variant of the multi-armed bandit is the {\em combinatorial multi-armed bandit} ~\cite{chenwei13}, in which a player sequentially explores a subset of arms (rather than a single arm), called a super-arm, that satisfies a certain combinatorial constraint.
% A different line of research on combinatorial bandits considers adversarial setting,
% in which a forecaster chooses a vector from a given finite set and an opponent chooses a “loss” vector to defeat the learning process~\cite{Cesa2012}.

% Another important variant of the multi-armed bandit is the {\em linear bandit}~\cite{Auer03}, where the expected reward is linear in the feature vector.
% In the linear bandit,
% for a dimension $m>0$, a player has the set of arms $D \subseteq \mathbb{R}^m$, called a \emph{decision set}.
% At each round $t$,
% the player pulls an arm $x \in {\cal D}$, and then observes a reward
% $r_t = x^{\top}\theta_* + \eta_t $, where $ \theta_* \in \mathbb{R}^m$ is an unknown parameter and $\eta_t$ is a zero-mean noise satisfying regularity conditions on the tail distribution.
% It should be noted that the linear bandit is a generalized model of the ordinary multi-armed bandit and combinatorial multi-armed bandit.
% When $D=\{e_1,e_2,\ldots,e_m\}$ 
% where $e_1,e_2,\ldots,e_m$
% are standard basis of the $m$-dimensional Euclidean space,
% %are the unit vectors in the standard Euclidean basis,
% linear bandits reproduce the ordinary multi-armed bandit.
% When $D \subseteq \{0,1\}^m$ represents a combinatorial action set, 
% the linear bandit coincides with 
% the combinatorial multi-armed bandit with a linear reward function 
% since each arm (and super-arm) can be represented by a feature $x \in \{ 0,1\}^m$. 



% \subsection{Best arm identification}
% In the literature of best arm identification problems,
% there are two different setting: {\em fixed confidence} and {\em fixed budget} setting defined as follows. Let {\tt Out} be an output of an algorithm and $i^*$ be an optimal arm.

% \begin{itemize}

%  \item  The fixed confidence setting:
% The learner need to guarantee that $\Pr[{\tt Out}=i^*] \geq 1-\delta$ for given confidence parameta $\delta$. The learner's performance is evaluated by her {\em sample complexity}, i.e. number of pulls used by the leaner.

%  \item The fixed budget setting:
% The leaner need to minimize the {\em probability of error}, which is formally $\Pr[{\tt Out} \neq i^*]$, within fixed number $T$ rounds.
   
% \end{itemize}

% In our work,
% Problem~\ref{prob:graph} corresponds to {\em fixed confidence} setting of PAC leaning.
% Problem~\ref{prob:graph_fixbudget} corresponds to {\em fixed budget} setting where the output is an approximate solution.

% %\paragraph{Best arm identification in linear bandits.}
% In the literature of best arm identification
% several researches studied the fixed confidence setting for linear bandits~\citep{Soare2014, Tao2018, Xu2018}.
% The top-$k$ arms identification problems have been also considered in the case where each individual arms can be queried or the learner obtains feedback from each arm in pulled subset of arms, i.e., {\em semi-bandit}~(e.g.~\cite{ bubeck2013, Gabillon2012}).

% Recently, combinatorial pure exploration problems have received increasing attention in the literature~\cite{Chen2014,Chen17a}
% A notable work for combinatorial pure exploration problems is \citet{Chen2014}
% that considered the case where reward function is linear objective under general setting, i.e., matroids, paths or matchings. In their work, they proposed combinatorial lower upper confidence bound algorithm (CLUCB) for the fixed confience setting and sucesseive accept reject algorithm (CSAR) for the fixed budget setting.
% Note that those algorithms cannot be directly used to solve our DS bandit problem because of non-linearity even in the case of semi-bandit setting or where each base arm can be queried at any round.
% In their setting, the learner aims to find the size-$k$ subset with maximal weights,
% while in ours, she aims to find any size of solution with maximal quality function.
% There are very few results on non-linear reward function even for a special case~\cite{huang2018}. 

% For the full-bandit case in which the only a noisy observation of the total sum of a subset is given at each pull, \citet{Idan2019} and \citet{Kuroki+19} proposed polynomial time algorithms for top-$k$ arms identification problem in the fixed confidence setting.
% However, in our case, we do not know the size of optimal subset in terms of both vertices and edges.
% When the size $k$-vertex is fixed in our case,
% the offline problem (called the densest $k$-subgraph problem) becomes
% NP-hard and the best known approximation ratio is $\Omega(1/n^{{1/4}+\epsilon})$ for any $\epsilon>0$~\cite{Bhaskara+10} as reviewed in Appendix~\ref{sec:related}.
% Note that the case where the fixed size $k$-edges is not meaningful in our problem,
% because top-$k$ edges does not mean the optimal subset of edges $E(S^*)$.


%We describe a general approach for solving the best arm identification problem in the linear bandit. 
% The basic idea is to construct a {\em confidence bound}, 
% which prescribes the uncertainty of the estimated reward of arms.
% The confidence interval should be constructed so that it contains the true parameter $\theta_*$ with high probability.
% %An algorithm sequentially pulls an arm and observes a reward sampled from an unknown distribution.
% To obtain the estimate of the unknown parameter $\theta_*$,
% the {\em least-squares estimator} $\widehat{\theta}_t$ is often used,
% which can be derived from the collected data $(x_1, r_1),\ldots,(x_t, r_t)$ such that $r_t \approx x_t^{\top}\theta_{*}$.
% % We stack them into matrices: $X_{1:t} \in t \times m$ and $Y_{1:t} \in m \times 1$. 
% % Then, we obtain the least-squares estimator $\widehat{\theta}_t$ defined as follows:
% % \[
% % \widehat{\theta}_t=(X_{1:t}X_{1:t}^{\top})^{-1}X_{1:t}^{\top}Y_{1:t}.
% % \]
% We maintain the confidence intervals,
% which the least-square estimator $\widehat{\theta}_t$ is the center of.
% Note that we need to pull arms so that confidence intervals will contain the parameter $\theta_*$ as soon as possible.
% To guarantee that the output is (nearly) optimal arm, 
% the algorithm checks a certain condition called the \emph{stopping condition}. 
% If the condition is true, then the algorithm outputs the empirical best arm $\widehat{x}^* =\argmax_{x \in \mathcal{D}}x^{\top} \widehat{\theta}_t$; otherwise the algorithm continue pulling arms. 


% We can recapture Problem~\ref{prob:graph} in the context of multi-armed bandit. 
% Each edge corresponds to an arm. 
% Each subset of edges $E(S)$ for $S\subseteq V$ corresponds to a super-arm. 
% To design our algorithm for Problem~\ref{prob:graph}, we utilize the approach based on linear bandit,
% in which we express a subset of edges $E(S)$ for $S\subseteq V$ as an arm whose feature is an indicator vector of it. 



\section{LP based exact algorithm for the densest subgraph problem}\label{sec:exact}

We describe an exact algorithm for the densest subgraph problem based on the following LP and simple rounding procedure proposed by ~\citet{Charikar2000} which we use in our proposed algorithm.

\begin{alignat}{4}\label{prob:lp} 
& &\ \ &\text{maximize} & \  & \sum_{e \in E} w_e x_e   \notag \\
&              &    &\text{subject to} &    &  x_e \geq y_u,\  x_e \geq y_v \ \   & \forall e= \{ u,v\} \in E, \notag \\
&              &    &  &    & \sum_{v \in V}y_v =1, & \notag \\
&              &    & &    & x_e, y_v \geq 0 & \forall e \in E, \forall v \in V. 
\end{alignat}

Let $(x^*, y^*)$ be an optimal solution to the above LP.
For a real number $r \geq 0$,
the algorithm considers a sequence of subsets vertices $S(r)=\{ v \in V \mid y^*_v \geq r\}$
and finds $r^*=\argmax_{r \in [0,1]}$.
Such a $r^:$ can be obtained by simply examining $r=y^*_v$ for each $v \in V$.
Finally, the algorithm outputs $S(r^*)$.
\citet{Charikar2000} proved that the output $S(r^*)$ is an optimal solution to the densest subgraph problem.


\section{Arm allocation strategy}\label{apx:allocation}

In this section, we introduce a possible allocation strategy that can be used in {\tt DS-Lin} algorithm.
To reduce the number of samples,
good arm allocation strategy makes confidence bound shrinking fast.
This suggests that an allocation strategy minimizing  $\max_{x \in \{0,1\}^m} \| x \|_{\Atin}$ reduced an optimal value of $\mathrm{P1}$ in the stopping condition~\eqref{stop}.
Thus,
we define the G-allocation in our setting as:
\[
p^G =\argmin_{p \in {\mathcal P}}\max_{x \in \{0,1\}^m} \| x \|_{\Lambda_p}.
\]
 There are existing studies that proposed approximate solutions
 to solve it in the experimental design literature ~\citep{mustapha2010, SAGNOL2013};
we can solve a continuous relaxation of the problem by a projected gradient algorithm.
For details on G-allocation or standard G-optimal design, see~\citet{Soare2014} or see~\citet{pukelsheim2006}.

%W mention the arm selection strategies in the multi-armed bandit.  
In general, an algorithm that adaptively changes an arm selection strategy based on the past observations at each round, which is called an {\em adaptive algorithm}, 
is desired because samples should be allocated for comparison of near-optimal arms in order to reduce the number of samples.
On the other hand,
the algorithm that fixes all arm selections before observing any reward is called the {\em static algorithm}.
Although the static algorithm is not able to focus on estimating near-optimal arms,
it can be used to analyze the worst case optimality.
In our text, each arm corresponds to an edge set; it is rare that any set is able to query since the possible choices are exponential.
Therefore, we design a static algorithm \textsf{DS-Lin} for solving Problem~\ref{prob:graph}.
On the other hand,  if we are allowed to query any action as in Problem~\ref{prob:graph_fixbudget}, we can design an adaptive algorithm \textsf{DS-SR}.


\section{Lower bounds for combinatorial pure exploration problems}\label{sec:lbound}
In the work of~\citet{Chen2014},
they proved that the lower bound on the sample complexity of general combinatorial pure exploration problems with linear rewards is $\Omega(\sum_{e \in [m]} \frac{1}{\Delta_{e}^2} \log \frac{1}{\delta})$, where $m$ is the number of base arms and $\Delta_e$ is defined as follows.
Let ${\cal M}$ be any decision class (such as size-$k$, paths, matchings, and matroids).
Let $M^*$ be the optimal subset, i.e., $M^*=\argmax_{M \in {\cal M}}\sum_{e \in M}w_e$.
For each base arm $e \in [m]$,
the gap $\Delta_e$ is defined as 
\[
  \Delta_e = \begin{cases}
    w(M^*) -\max_{M \in {\cal M} \mid e \in M} \sum_{e \in M}w_e & ({\rm if} \ e \notin M^* ) \\
    w(M^*)-\max_{M \in {\cal M} \mid e \notin M} \sum_{e \in M}w_e & ({\rm if} \ e \in M^* ).
  \end{cases}
\]



In the work of ~\citet{huang2018},
they studied the combinatorial pure exploration problem with continuous and separable reward functions, and showed that the problem have a lower bound $\Omega({\bf H_{\Lambda}} +{ \bf H_{\Lambda} } m^{-1} \log (  \delta^{-1}))$, where ${ \bf H_{\Lambda} }= \sum_{i=1^m} \frac{1}{\Lambda^2_i}$.
In their definition of ${ \bf H_{\Lambda} }$,
the term $\Lambda_i$ is called {\em consistent optimality radius} and it measures how far the estimate can be away from true parameta while the optimal solution in terms of the estimate is still consistent with the true optimal one in the $i$-th dimension (see Definition~2 in~\cite{huang2018}).

Note that the problem settings in~\citet{Chen2014} and ~\citet{huang2018} are different from ours, since in our setting the learner can query a subset of edges rather than a base arm and reward function is the average-degree in a given graph.
Therefore their lower bound results cannot directly apply to our problem.
However, we can see that our sample complexity in Theorem~\ref{thm:samplecomplexity} is comparable with them since ours is $O(\He \log \delta^{-1}+ \He \log(\He \log \delta^{-1}))$ if we ignore the terms not related to $\He$ and $\delta$.




\section{Technical Lemmas for Theorem~\ref{thm:samplecomplexity}}\label{apx:thm1}




% The following lemma shows that Algorithm~\ref{alg:sdp} admits a constant-factor approximation ratio for $\mathrm{P1}$.
% \begin{lemma}\label{lemma:approx}
% Algorithm~\ref{alg:sdp} is a $\sqrt{2/\pi}$-approximation algorithm for P1.  %in~\eqref{prob:CBM}.
% \end{lemma}



% %\section{Proof of Lemma~\ref{lemma:approx}}

% % \begin{lemma}
% % Algorithm~\ref{alg:sdp} is a $\sqrt{2/\pi}$-approximation algorithm for P1.  %in~\eqref{prob:CBM}.
% % \end{lemma}

% \begin{proof}
% % Solving the problem P1 is equivalent to the unconstrained binary quadratic programming $\mathrm{P2}$.
% %Nesterov~\cite{Nestrov1998} showed that an SDP-based algorithm gives a $2/\pi$-approximate solution for P2 in Algorithm~\ref{alg:sdp}. %the the following quadratic programming: 
% %\begin{alignat*}{8}%\label{prob:CBM} %Jo:alignat*なのでラベルが貼られない
% %& &\ \text{P2:} \ &\text{maximize} & \sum_{1 \leq i, j \leq m }q_{ij}x_ix_j &&&  \\
% %& &    &\text{subject to} \ \ \ &x_i \in \{-1,+1\} &&& \ \ \text{for all}\  i=1, \ldots, m.
% %\end{alignat*}
% %where the objective function matrix $Q=(q_{ij})$ is positive semidefinite.
% %Now we will show that P1 admits $\sqrt{2/\pi}$-approximation by Algorithm~\ref{alg:main}.
% %which is based on the algorithm based on semidefinite programming and rounding procedure for the unconstrained binary quadratic programming $\mathrm{P2}$ proposed in Nestrov~\cite{Nestrov1998}.
% %We first review that Nesterov's algorithm~\cite{Nestrov1998} is a $2/\pi$-approximation algorithm for P2.

% We denote the inner product of $v_i \in \mathbb{R}^m$ and $v_j \in \mathbb{R}^m$ as $v_i \cdot v_j$.
% Then, we have the following SDP relaxation for P2: 
% \begin{alignat*}{8}%\label{prob:CBM} 
% & \text{SDP:}  &\ &\text{maximize}   &\ \ &\sum_{1 \leq i, j \leq m }q_{ij}(v_i \cdot v_j)\\
% &              &  &\text{subject to} &    &v_i \cdot v_i =1     &&\hspace{-8mm} \text{for all}\ i=1, \ldots, m, \\
% &              &  &                  &    &v_i \in \mathbb{R}^m &&\hspace{-8mm} \text{for all}\ i=1, \ldots, m.
% \end{alignat*}
% This relaxation can be solved in polynomial time and we obtain vectors $(v_i)_{i, \ldots, m}$.
% In Nesterov's algorithm~\cite{Nestrov1998},
% we choose a random hyperplane with normal $\ell$,
% and then construct a solution $\overline{x}$ for P2 by rounding $\overline{x}_i=1$
% if $\ell \cdot v_i \geq 0$ and $\overline{x}_i=-1$ otherwise. 
% This rounding procedure results in a $\frac{2}{\pi}$-approximation algorithm for P2.
% We can convert P2 in $\{-1, 1\}$ domain to
% the quadratic program P1 in $\{0, 1\}$ domain by setting $y_i=\frac{x_i+1}{2}$ for $i \in \{1,\dots, m\}$.
% Then, the objective function becomes as follows:
% \[4\sum_{1 \leq i, j \leq m }q_{ij}y_iy_j + 2\sum_{1 \leq i, j \leq m}q_{ij}(y_i+y_j)+ \sum_{1 \leq i, j \leq m}q_{ij}.
% \]
% Since $Q$ is positive semidefinite, we have $\sum_{1 \leq i, j \leq m }q_{ij} \geq 0$.
% From the fact that the probability that $v_i$ and $v_j$ will be on different sides of the random hyperplane is $\frac{1}{\pi} \arccos(v_i \cdot v_j)$ (see \citet{Nestrov1998} for the detail),
% we see that
% \begin{alignat*}{4}
% \Pr[\overline{x}_i+\overline{x}_j=-2] &=\Pr[\overline{x}_i+\overline{x}_j=+2]\\
% &=\frac{1}{2}\left( 1-\frac{1}{\pi}\arccos{v_i \cdot v_j}\right).
% \end{alignat*}
% From the equation, we have $\Exp[y_i+y_j]=0$.
% This implies that the approximation ratio ${\frac{2}{\pi}}$ is kept for P2 in $\{0, 1\}$ domain,
% since Nesterov's algorithm gives ${\frac{2}{\pi}}$-approximation for P2 in $\{-1, 1\}$ domain.
% Hence, Algorithm~\ref{alg:main} gives $\sqrt{\frac{2}{\pi}}$-approximation for P1, since $\Atin$ is also positive semidefinite.
% \end{proof}




Next,
we introduce random event $\cE_t$ which characterizes
the event that the confidence bounds of
any feasible solution $ S \in V$
are valid at round $t$.
 We define a random event $\cE_t$ as follows:
 \begin{alignat}{4}\label{event}
&{\cal E}_t=\{ \forall S \in V \ {\rm and }  \  v \in S, 
  &\quad  \left| w(S)-\widehat{w}_t(S) \right| \leq C_t \| \chiEofS  \|_{\Atin} \}.
\end{alignat}

The following lemma states that event $\cE=\bigcap_{t=1}^{\infty} \cE_t$ occurs with high probability.
\begin{lemma}\label{lemma:highprob}
 The event ${\cal E} $ occurs with probability at least $1-\delta$.
\end{lemma}
The proof is omitted since it is straightforward from Proposition~1 and union bounds.



\begin{lemma}\label{lemma:epsilonoptimal}
For a fixed round $t > m$,
assume that $\cE_t$ occurs.
Then, if the algorithm stops at round $t$, the output of the algorithm $S_{\tt OUT}$ satisfies $f_w(S^*)-f_w(S_{\tt OUT})  \leq \epsilon$.
%with probability at least $1-\delta$.
\end{lemma}

\begin{proof}



% \begin{align}\label{stop}
% f_{\widegat{w}_t}(\widehat{S}_t)- \frac{C_t \|\chiEofShat \|}{|\widehat{S}_t|} \geq \max_{ S \neq \widehat{S}_t \mid S \subseteq  V}f_{\widehat{w}_t}(S)+ \frac{Z_t}{2 \alpha } -\epsilon,
% \end{align}

If $S_{\tt OUT}= S^*$, we obviously have the desired result.
Then, we shall assume $S_{\tt OUT} \neq S^*$.
\begin{alignat*}{5}
f_w(S_{\tt OUT}) & \geq f_{w_t}(S_{\tt OUT})-\frac{C_t \normAhatstar }{| S_{\tt OUT}| } \\ \notag
&\geq 
\max_{ S \neq S_{\tt OUT} \mid S \subseteq  V}f_{\widehat{w}_t}(S)+ \frac{C_t Z_t}{2 \alpha } -\epsilon \\ \notag
&\geq 
f_{\widehat{w}_t}(S^*)+ \frac{ \max_{x \in \{0,1\}^m} \| x \|_{\Atin}}{2 } -\epsilon \\ \notag
&\geq 
f_{\widehat{w}_t}(S^*)+ \frac{ \max_{S \subseteq V} \| \chiEofS \|_{\Atin}}{2 } -\epsilon \\ \notag
&\geq  f_{\widehat{w}_t}(S^*) +\frac{C_t \| \chiEofSstar\|}{|S^*|}-\varepsilon  \hspace{0.8cm}
\\\notag
&\geq  f_w(S^*)-\varepsilon,
\end{alignat*}
where the first and last inequalities follow from the event $\cE_t$,
and the second inequality follows from the stopping condition,
and the third inequality follows from the definition of $Z_t$ and approximation ratio $\alpha$.
\end{proof}

In \citet{Miyauchi_Takeda_18},
they provided the following lemma, which we also use to prove Theorem~\ref{thm:samplecomplexity}.
\begin{lemma}[\citet{Miyauchi_Takeda_18}, Lemma~2]\label{lemma:miyauchi}
Let $G=(V,E)$ be an undirected graph.
Let $w_1$ and $w_2$ be edge-weight vectors such that $\| w_1-w_2\|_{\infty} \leq \beta$ holds for $\beta>0$.
Then, for any $S \subseteq V$, it holds that
\[
|f_{w_1}(S)-f_{w_2}(S) | \leq \sqrt{\frac{m}{2}} \cdot \beta.
\]
\end{lemma}



\section{Proof of Theorem~\ref{thm:samplecomplexity}}








\begin{proof}
We know that the event $\cE$ holds with probability at least $1-\delta$ from Lemma~\ref{lemma:highprob}.
Therefore, we only need to prove that, under event $\cE$,
the algorithm returns a set whose density is at least $f_w(S^*)-\epsilon$ and provide an upper bound of number of queries.
From Lemma~\ref{lemma:epsilonoptimal},
on the event $\cE$, the algorithm outputs $S_{\tt OUT} \subseteq V$ that satisfies $f_w(S^*)-f_w(S_{\tt OUT}) \leq \epsilon$.

Next, we focus on bounding the number of queries.
Recall that Algorithm~\ref{alg:main} employs a  stopping condition:
\begin{align}
&f_{\widehat{w}_t}(\widehat{S}_t)- \frac{C_t \|\chiEofShat \|}{|\widehat{S}_t|} \geq \max_{ S \neq \widehat{S}_t \mid S \subseteq  V}f_{\widehat{w}_t}(S)+ \frac{C_t Z_t}{2 \alpha } -\epsilon,
\end{align}
where $Z_t$ denotes the objective of the  approximate solution to P1.  %in~\eqref{prob:CBM},
% and the stopping condition guarantees us
% to have
% $\epsilon \geq C_t \max_{S \subseteq V, v \in S}  \| \chiEofSv\|_{\At^{-1}}$.
% This bound gives $|\text{deg}_S(v,w)-\text{deg}_S(v,\widehat{w}_{t})| \leq \epsilon$ for any set $S \subseteq V $ and $v \in S$ 
% under the event $\cE$.
% By 
% %Lemma~\ref{lemma:highprob}
% %~\eqref{epsilonoptimal}
% Theorem~\ref{thm:approx},
% we see that the output $\widehat{S}^*$ has the objective value at least $\frac{f_w(S^*)}{2}-\epsilon $.
%with probability at least $1-\delta$.
A sufficient condition of the stopping condition is that for $S^*$ and for $t >m$,
\begin{align}
    f_{\widehat{w}_t}(S^*)- \frac{C_t \| \chiEofSstar \|}{ | S^* |} \geq  \max_{S \neq S^* \mid S \subseteq V }f_{\widehat{w}_t}(S) + \frac{C_t Z_t}{2\alpha}-\epsilon,
\end{align}
%where recall that $\alpha= \sqrt{\frac{\pi}{2}}$ from Lemma~\ref{lemma:approx}.
Since $Z_t \leq \max_{x \in \{0,1\}^m} \|x \|_{\Atin}  $ and $\| \chiEofSstar \| \leq \max_{x \in \{0,1\}^m} \|x \|_{\Atin}$,
the following inequality is also a sufficient condition to stop:
\begin{align}\label{ineq:suf1}
        f_{\widehat{w}_t}(S^*)- \frac{C_t \max_{x \in \{0,1\}^m} \|x \|_{\Atin} }{ | S^* |} \geq  \max_{S \neq S^* \mid S \subseteq V }f_{\widehat{w}_t}(S) + \frac{ C_t \max_{x \in \{0,1\}^m} \|x \|_{\Atin} }{2\alpha}-\epsilon.
\end{align}
Recall that  $T_t(S)$ be the number of times that $S \subseteq {\cal S}$ is queried before $t$-th round in the algorithm.
We denote $p_{\bf{x}_t} $ by $ p_{\bf{x}_t} =(T_t(S)/t)_{S \in \mathcal{S}}$.
From the above definitions, the design matrix is $\At= t \Lambda_{p_{\bf{x}_t}}$. 
Recall that $\rho_{\Lambda_p}=\max_{x \in \{0,1\}^m} \|x \|^2_{ {\Lambda^{-1}_p}}$,
and let $\rho_{\Lambda_{p_{\bf{x}_t}}}=\max_{x \in \{0,1\}^m} \|x \|^2_{{\Lambda^{-1}_{p_{\bf{x}_t}}}}$.
From the fact that $ \lim_{t \to \infty}\Lambda_{p_{\bf{x}_t}} =\Lambda_p $,
for sufficiently large $t \gg m$  we have that $ |\rho_{\Lambda_p} -\rho_{\Lambda_{p_{\bf{x}_t}}}| \leq \epsilon$ with probability at least $1-\frac{\delta}{2}$ where $\delta \in (0,1)$ and $\epsilon>0$.
Let $ \bar{S}=\argmax_{S \neq S^* \mid S \subseteq V }f_{\widehat{w}_t}(S)$.
Then, \eqref{ineq:suf1} is rewritten as follows:
\begin{align}\label{ineq:suf2}
     f_{\widehat{w}_t}(S^*)-f_{\widehat{w}_t}(\bar{S}) \geq \left( \frac{1}{|S^*|}+ \frac{1}{2\alpha}  \right) C_t \sqrt{ \frac{\rho_{\Lambda_p} + \epsilon}{t} } -\epsilon.
\end{align}

Next, we show the following inequality.
\begin{align}\label{ineq:rhs_lower}
   f_{\widehat{w}_t}(S^*)-f_{\widehat{w}_t}(\bar{S}) \geq  \Delta_{\min}-\sqrt{2m} C_t \sqrt{ \frac{\rho_{\Lambda_p}+\epsilon}{t} }.
\end{align}
From Proposition~\ref{propo:yadokori}, with probability $1-\frac{\delta}{2}$,
we have  $\| w- \widehat{w}_t  \|_{\infty} \leq C_t \max_{S} \| \chiEofS \|_{\Atin}$.
% In Miyauchi and Takeda~\cite{Miyauchi_Takeda_18},
% they provided the following lemma.
% \begin{lemma}[Miyauchi and Takeda~\cite{Miyauchi_Takeda_18}, Lemma~2]\label{lemma:miyauchi}
% Let $G=(V,E)$ be an undirected graph.
% Let $w_1$ and $w_2$ be edge-weight vectors such that $\| w_1-w_2\|_{\infty} \leq \beta$ holds for $\beta$ >0.
% Then, for any $S \subseteq V$, it holds that
% \[
% |f_{w_1}(S)-f_{w_2}(S) | \leq \sqrt{\frac{m}{2}} \cdot \beta.
% \]
% \end{lemma}
From Lemma~\ref{lemma:miyauchi},
we see that $f_{\widehat{w}_t}(S^*)-f_w(S^*) \geq - \sqrt{\frac{m}{2}} C_t \max_{S \subseteq V} \| \chiEofS\|_{\Atin}$ and $f_w(\bar{S})-f_{\widehat{w}_t}(\bar{S}) \geq - \sqrt{\frac{m}{2}} C_t \max_{S \subseteq V} \| \chiEofS\|_{\Atin}$.
Therefore,
for sufficiently large $t \gg m$ such that $ |\rho_{\Lambda_p} -\rho_{\Lambda_{p_{\bf{x}_t}}}| \leq \epsilon$ with probability at least $1-\frac{\delta}{2}$, we have that
\begin{alignat*}{4} 
f_{\widehat{w}_t}(S^*)-f_{\widehat{w}_t}(\bar{S}) & \geq f_w(S^*)-f_w(\bar{S})-\sqrt{2m} C_t  \max_{S \subseteq V} \| \chiEofS \|_{\Atin} \\
& \geq f_w(S^*)-f_w(\bar{S})-\sqrt{2m} C_t  \max_{x \in \{0,1\}^m } \| x \|_{\Atin} \\
& = f_w(S^*)-f_w(\bar{S})-\sqrt{2m} C_t \sqrt{ \frac{\rho_{\Lambda_{p_{\bf{x}_t}}}}{t} }\\ 
& \geq f_w(S^*)-f_w(\bar{S})-\sqrt{2m} C_t \sqrt{ \frac{\rho_{\Lambda_p}+\epsilon}{t} }\\
& \geq  \Delta_{\min}-\sqrt{2m} C_t \sqrt{ \frac{\rho_{\Lambda_p}+\epsilon}{t} }.
\end{alignat*}
Then, we obtain \eqref{ineq:rhs_lower}.
Combining \eqref{ineq:suf2} and \eqref{ineq:rhs_lower},
we see that the following inequality is a sufficient condition to stop:
\begin{align}\label{ineq:suf3}
    \Delta_{\min}-\sqrt{2m} C_t \sqrt{ \frac{\rho_{\Lambda_p}+\epsilon}{t} } \geq \left( \frac{1}{|S^*|}+ \frac{1}{2\alpha}  \right) C_t \sqrt{ \frac{\rho_{\Lambda_p}+\epsilon}{t} } -\epsilon.
\end{align}
Solving \eqref{ineq:suf3} with respect to $t$,
we obtain 
\begin{align}
    t \geq (\sqrt{2m} + |S^*|^{-1} + 2\alpha^{-1})^2 C_t^ 2 \He,
\end{align}
where recall that $\He$ is defined as 
\begin{align*}
    \He= \frac{ \rho_{\Lambda_p}+\epsilon }{ (\Delta_{\min} + \epsilon)^2}.
\end{align*}


% A sufficient condition to hold the stopping condition $\epsilon \geq C_t Z_{t}$
% is
% the following inequality: 
% \begin{align}\label{eq:stop2}
% \epsilon' \geq  C_t  \max_{x \in \{0,1\}^m} \|x \|_{\Atin},
% \end{align}
% since trivially $Z_t \leq \max_{x \in \{0,1\}^m} \|x \|_{\Atin} $.
% From the definition of $\Lambda_t$ and $\Lambda({\cal S})$,
% we see that $\text{E}[\Lambda_t]=\Lambda({\cal S})$.
% % ${\Lambda_p}=\frac{1}{| \mathcal{S}|}\sum_{S \in \mathcal{S}} \chiEofS \chiEofS^{\top}$ and  $ \rho_\Lambda=\max_{x \in \{0,1\}^m} \|x \|^2_{\Lambda_p}$.
% Recall that $\rho_\Lambda=\max_{x \in \{0,1\}^m} \|x \|^2_{\Lambda({\cal S})^{-1}}$.
% Then, \eqref{eq:stop2} is written as
% \begin{align}
% \epsilon' \geq  C_t\sqrt{\frac{\rho_\Lambda}{t }},
% \end{align}
% where recall that $\At=\sum_{i=1}^t \bm{\chi}_{\sm {$E(S_t)$}}\bm{\chi}_{\sm {$E(S_t)$}}^{\top} +\lambda I $.
Therefore, from the above, we obtain $ t \geq  \left(\sqrt{2m} + |S^*|^{-1} + {2\alpha}^{-1} \right)^2 C_t^ 2 \He$ as a sufficient condition to stop.
Let $\tau >m$ be the stopping time of the algorithm.
From the above discussion and $|S^*| \geq 2$,
we see that 
\begin{align}\label{ineq:uppre_tau}
    \tau \leq  \left(\sqrt{2m} + \frac{\alpha+1}{2}\right)^2 C_\tau^ 2 \He.
\end{align}
Now we bound $C_{\tau}$ in~\eqref{ineq:uppre_tau}.
We have $\det(\Atau) \leq (\lambda + \tau )^m$,
 which is obtained by Lemma~10 in \citet{yadkori11}.
Then,
we obtain the following inequality in the similar manner in Theorem 2 in \citet{Xu2018}:
\begin{alignat}{4}\label{ineq:ctbound}
C_{\tau}& \leq  R' \sqrt{2 \log \frac{\det(\Atau)^{\frac{1}{2}} \det(\lambda  I)^{-\frac{1}{2}}}{\delta} } +\lambda^{\frac{1}{2}}L \notag \\
& \leq  R' \sqrt{2 \log \frac{1}{\delta}       
+ m \log \left( 1+ \frac{\tau}{\lambda}  \right)
}+\lambda^{\frac{1}{2}}L.
\end{alignat}

Using~\eqref{ineq:ctbound}, we give an upper bound of $\tau$.
We also use a similar proof strategy as in \citet{Xu2018}.
First, let us consider the case $\lambda>4 m(\sqrt{m}+\sqrt{2})^2  R'^2 \He$, where recall that $R'=\sqrt{ \text{deg}_{\max}}R$.
Using the facts that $(a+b)^2 \leq 2(a^2+b^2)$ for $a,b>0$ and $\log (1+x) \leq x$,
we have 
\begin{alignat*}{4}
\tau & \leq \left(\sqrt{2m} + \frac{\alpha+1}{2}\right)^2 C_{\tau}^2 \He 
 \leq 2\left(\sqrt{2m} + \frac{\alpha+1}{2}\right)^2\He \left(  4 R'^2  \log \frac{1}{\delta} +\frac{R'^2 m }{\lambda}\tau  +\lambda L^2 \right).
\end{alignat*}
Thus, we obtain
\begin{alignat*}{4}
\tau & \leq \left( 1-2\left(\sqrt{2m} + \frac{\alpha+1}{2}\right)^2 \frac{R'^2 m \He}{\lambda} \right)
^{-1} ( 8 \He R'^2 \log 1/ \delta +2\He \lambda L^2 ) \\
& \leq 2 (8 \He R'^2 \log 1/ \delta +2\He \lambda L^2 ),
\end{alignat*}
where the last inequality holds from $\lambda>4 m(\sqrt{m}+\sqrt{2})^2  R'^2 \He$ and $\alpha=\sqrt{\frac{2}{\pi}}$.
Therefore, in this case,
we obtain 
\[
\tau=O \left(\left(\text{deg}^2_{\max} R^2 \log \frac{1}{\delta}+ \lambda L^2 \right)  \He \right).
\]

Second, we consider $\lambda \leq  \frac{R'^2}{L^2} \log \left(\frac{1}{\delta}\right)$.
From this bound and~\eqref{ineq:ctbound},
we have
\begin{alignat*}{4}
C_{\tau}& 
%\leq R' \sqrt{ 2 \log(1)/\delta + m \log \left( 1+ \frac{ \tau}{\lambda}\right)  } +\lambda^{\frac{1}{2}}L\\
%& 
\leq  2R' \sqrt{ 2 \log \frac{1}{\delta} + m \log \left( 1+ \frac{ \tau}{\lambda} \right) }.
\end{alignat*}
Let $V(m, \alpha)=\left(\sqrt{2m} + \frac{\alpha+1}{2}\right)^2$.
Therefore,
we obtain
\begin{alignat*}{4}
\tau & \leq V(m, \alpha) C_{\tau}^2\He 
\leq 4 V(m, \alpha) R'^2 \left( 2 \log \frac{1} {\delta}   + m \log \left( 1+\frac{ \tau}{\lambda}  \right)\right) \He.
\end{alignat*}
Let $N=8  V(m, \alpha)R'^2 \log  \frac{1} {\delta}  \He$ and let $\tau'$ be a parameter satisfying:
\begin{align}\label{parameta_tauprime}
    \tau =  N
+ 4V(m, \alpha)R'^2 m \log \left( 1+\frac{ \tau'}{\lambda}  \right)\He.
\end{align}
It is easy to see $\tau'  \leq \tau$.
Then, we have 
\begin{alignat*}{3}
\tau'  &\leq \tau =N+ 4V(m, \alpha)  R'^2 m \log \left( 1+\frac{ \tau'}{\lambda}  \right) \He\\
& \leq N+ 4 V(m, \alpha)R'^2 m  \sqrt{\frac{\tau'}{\lambda}} \He,
\end{alignat*}
where the second inequality follows from the fact $\log (1+x) \leq \sqrt{x}$.
Solving this quadratic inequality for $\sqrt{\tau'}$,
 we have
 \begin{alignat}{4}\label{tauprimebound}
 \sqrt{\tau'}& \leq \frac{2 V(m, \alpha)R'^2 m \He}{\sqrt{\lambda}}+
 \sqrt{ \frac{4V(m, \alpha)^2  R'^4 m^2 \He^2 }{\lambda} + N} \notag\\
 &\leq 2 \sqrt{ \frac{4 V(m, \alpha)^2 R'^4m^2 \He^2}{\lambda} +N}.
\end{alignat}
Let $M=2 \sqrt{ \frac{4 V(m, \alpha)^2R'^4m^2 \He^2 }{\lambda} +N}$.
We can give an upper bound $\tau$ by~\eqref{parameta_tauprime} and~\eqref{tauprimebound} as follows:
\begin{align*}
    \tau \leq 8 V(m, \alpha)R'^2 \He \log \frac{1}{\delta} + 4 \He V(m, \alpha)R'^2 m \log \left( 1+\frac{M}{\lambda} \right).
\end{align*}

Note that $\log M= O\left( \log \left( R'^4m^4 \He^2 + m R'^2 \log \frac{1}{\delta}\He   \right) \right)$ since $ V(m, \alpha)=O(m)$.
From the above and $R'=\sqrt{\text{deg}_{\max}}R$,
we obtain
\begin{alignat*}{4}
\tau =  & O \left( m \text{deg}_{\max} R^2 \He \log \frac{1}{\delta} +m\text{deg}_{\max}  R^2 \He  \log \left(\text{deg}_{\max}^2 R^4 m^4 \He^2 + m \text{deg}_{\max}R^2 \He  \log \frac{1}{\delta} \right) \right)\\
& = O \left( m \text{deg}_{\max} R^2 \He \log \frac{1}{\delta}+C(\He, \delta) \right) 
\end{alignat*}
where 
\begin{alignat*}{4}
    & C(\He, \delta)=m\text{deg}_{\max}  R^2 \He  \log \left(\text{deg}_{\max}^2 R^4 m^4 \He^2 + m \text{deg}_{\max}R^2 \He  \log \frac{1}{\delta} \right) \\
    & = O\left( m\text{deg}_{\max}  R^2 \He  \log \left(\text{deg}_{\max} R m \He \log \frac{1}{\delta} \right) \right).
\end{alignat*}
% \begin{align*}
%     C(\He, \delta)=O\left( m\text{deg}_{\max}  R^2 \He  \log \left(\text{deg}_{\max} R m \He \log \frac{1}{\delta} \right) \right).
% \end{align*}
\end{proof}

\section{Technical Lemmas for Theorem~\ref{thm:fixbudget}}

First we introduce a standard concentration inequality of sub-Gaussian random variables~\cite{Chen2014}.
\begin{lemma}[\citet{Chen2014}, Lemma~6]\label{lemma:hoef}
Let $X_1, \ldots, X_k$ be $k$ independent random variables such that, for each $i \in [k]$, random variable $X_i- \mathbb{E}[X_i]$ is R-sub-Gaussian distributed, i.e., $\forall a \in \mathbb{R}$, $\mathbb{E}[\exp(aX_i-a \mathbb{E}[X_i])] \leq \exp(R^2a^2)/2$. 
Let $\bar{X}= \frac{1}{k} \sum_{i=1}^k X_i$ denote the average of these random variables.
Then, for any $\lambda >0$, we have
\[
\Pr \left[ |\bar{X}- \mathbb{E}[\bar{X}] | \geq \lambda \right] \leq 2 \exp \left( - \frac{k\lambda^2}{2R^2} \right).
\]

\end{lemma}


For $S\subseteq V$, $v\in S$, and expected weight $w$, 
we denote by $\text{deg}^*_S(v)$ the weighted degree of $v\in S$ on $G[S]$ in terms of the true edge weight $w$.
We show the following lemma used for analysis of Algorithm~\ref{alg:peeling_approxx2}.
\begin{lemma}\label{lemma:fix_budget_lemma}
Given an phase $t \in \{1,\ldots,n-1\}$, 
we define random event 
\begin{align}
    \mathcal{E}_t' = \left\{ \forall v \in S_{n-t+1}, \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v,t) \right| \leq \epsilon \right\}.
\end{align}
Then, we have 
\begin{align}
 \Pr   \left[  \bigcap_{t=1}^{n-1} \mathcal{E}_t' \right] \geq 1- \frac{2 \text{deg}_{\max} 2^n R^2}{\epsilon^2}(n+1)^3 \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max}  \tilde{ \log }(n-1) } \right).
\end{align}



\end{lemma}
\begin{proof}

For any $S \subseteq V$, and $v \in S$,
recall that $X_{E_S(v)}(i)$ is $i$-th observation of edge-weights $E_S(v)$
for $i \in [k]$.
Then,
$X_{E_S(v)}(i)- \mathbb{E}[X_{E_S(v)}(i)]$ follows $\sqrt{|E_S(v)|}R$ sub-Gaussian distribution.
% We have that  \[
% \bar{X} =\frac{\sum_{i=1}^k  r(E_S(v),i)}{k}=  \hat{r}(E_S(v),k) = \widehat{\text{deg}}_{S}(v,k),
% \]
% and \[
% \mathbb{E}[\bar{X}]=\mathbb{E} \left[  \sum_{i=1}^k  \sum_{e \in E_S(v)} w_e \right]/k +\sum_{i=1}^k \mathbb{E}\left[\sum_{e \in E_S(v)} \eta_e(i) \right]/k =\sum_{e \in E_S(v)} w_e= \text{deg}^*_{S}(v).
% \]
We can assume that the sequence of weights for each subset of edges is drawn before the beginning of the game.
Thus $\hat{X}_{E_S(v)}(k)$ is well defined even if $E_S(v)$ has not been actually sampled $k$ times.
Therefore, from Lemma~\ref{lemma:hoef},  for any $\epsilon >0$
we have that 
\begin{align}\label{ineq:hoeff_graph}
\Pr \left[  \left| \mathbb{E}[{\hat{X}_{E_S(v)}(k)}]- \hat{X}_{E_S(v)}(k)\right|  \geq \epsilon \right] \leq 2 \exp \left( - \frac{k\epsilon ^2}{2 |E_S(v)|R^2} \right) \leq  2 \exp \left( - \frac{k\epsilon ^2}{2  \text{deg}_{\max} R^2} \right) .    
\end{align}

% \begin{align}\label{ineq:hoeff_graph_2}
% \Pr \left[  \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v) \right|  \geq \epsilon \right] \leq 2 \exp \left( - \frac{k\epsilon ^2}{2 |E_S(v)|R^2} \right) \leq  2 \exp \left( - \frac{k\epsilon ^2}{2  \text{deg}_{\max} R^2} \right) .    
% \end{align}

% Let $\tilde{{\cal S}} = \{  S_1, S_2, \ldots, S_n  \}$.
% For $S_i \in \tilde{{\cal S}}$, we have
% \begin{alignat}{4}\label{ineq:prob_deg}
%  &\Pr \left[  \left| \text{deg}^*_{S_{i}}(v) - \widehat{\text{deg}}_{S_{i}}(v) \right| \geq \epsilon \right] \\
%  %& = \sum_{S \in 2^V} \Pr[S_{n-t+1}=S]  \Pr \left[  \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v) \right| \geq \epsilon   \middle| S_{n-t+1} =S \right] \\
%  & \leq \Pr \left[  \exists S \subseteq V  \middle| \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v) \right| \geq \epsilon  \right] \\
%   & \leq \sum_{ S \in \tilde{{\cal S}} } \Pr \left[ \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v) \right| \geq \epsilon    \right].
% %     & \leq \sum_{S \in 2^V } \Pr \left[  \exists S \subseteq V \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v) \right| \geq \epsilon    \right] \\
% %   & \leq \sum_{S \in 2^V } 2 \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{8n^3 |E_{S_{n-t+1}}(v)|R^2 \tilde{ \log }(n-1)   } \right)\\
% %   & = 2^{n+1}\exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{8n^3 |E_{S_{n-t+1}}(v)|R^2 \tilde{ \log }(n-1)   } \right)
%   \end{alignat}
  
  Fix $t \in \{ 1,\ldots, n-1 \}$ and fix a vertex $v \in S_{n-t+1}$ in a phase $t$.
% For all $t \in \{ 1,\ldots, n-1 \}$ and a vertex $v \in S_{n-t+1}$ such that 
If $|N_{S_{n-t+1}}(v)| =0$, it is obvious that $ \text{deg}_{S_{n-t+1}}(v) =\widehat{\text{deg}}_{S_{n-t+1}}(v) =0$.
Therefore, we will consider a vertex $v \in S_{n-t+1}$ such that $|N_{S_{n-t+1}}(v)| \geq 1$ in the rest of the proof.
  By the definition of $\tilde{T}_t$ for $t \in [ 1,2, \ldots, n-1]$,
  we have $\tilde{T}_t \geq \frac{T-\sum_{i=1}^{n+1}i}{(n-t) \tilde{\log}(n-1)} \geq \frac{T-\sum_{i=1}^{n+1}i}{n \tilde{\log}(n-1)}$.
 % Notice that $E_{S_{n-t+1}}(v)$ has been sampled for $T'_t$ times during the first $t$ phase, since at each phase $t$ the algorithm samples $E_{S_{n-t+1} \setminus \{u\}}(v)$ for $u \in N_{S_{n-t+1}(v)}$.
 Then for $T_{E_{S_{n-t+1}}(v)}(t)$, we have:
\begin{align}\label{ineq:times}
T_{E_{S_{n-t+1}}(v)}(t)  = \sum_{i=1}^t \tau_i
=\sum_{i=1}^t (T_i'- T'_{i-1}) 
= T_t'  
\geq \frac{\tilde{T}_t}{2|S_{n-t+1}|}
\geq  \frac{T-\sum_{i=1}^{n+1}i}{ 2n^2\tilde{\log}(n-1)}.
\end{align}

Let $k'$ be the RHS of ~\eqref{ineq:times}, i.e. $k' =\frac{T-\sum_{i=1}^{n+1}i}{ 2n^2\tilde{\log}(n-1)}$.
For $v \in S_{n-t+1}$, we have
\begin{alignat}{4}\label{ineq:deg}
 &\Pr \left[  \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v,t) \right| \geq \epsilon \right] \notag \\
  & =\Pr \left[  \left| \mathbb{E}[{\hat{X}_{E_{S_{n-t+1}}(v)}(T_{E_{S_{n-t+1}}(v)}(t))}]- \hat{X}_{E_{S_{n-t+1}}(v)}(T_{E_{S_{n-t+1}}(v)}(t))\right|  \geq \epsilon \right] \notag \\
  &\leq \Pr \left[  \exists S \subseteq V, u \in S \middle| \left| \mathbb{E}[{\hat{X}_{E_{S}(u)}(T_{E_{S_{n-t+1}}(v)}(t))}]- \hat{X}_{E_{S}(u)}(T_{E_{S_{n-t+1}}(v)}(t))\right| \geq \epsilon  \right]  \notag \\
&\leq \sum_{S \in 2^V}  \sum_{ u \in S}　\sum_{k=k'}^{\infty} \Pr \left[ \left| \mathbb{E}[{\hat{X}_{E_{S}(u)}(k)}]- \hat{X}_{E_{S}(u)}(k)\right| \geq \epsilon  \right]  \notag \\
& \leq \sum_{S \in 2^V}  \sum_{ u \in S}　\sum_{k=k'}^{\infty} 2 \exp \left( - \frac{k\epsilon ^2}{2  \text{deg}_{\max} R^2} \right) \notag \\
& = \sum_{S \in 2^V}  \sum_{ u \in S}　\frac{ 2 \exp \left( - \frac{k'\epsilon ^2}{2  \text{deg}_{\max} R^2} \right) }{\exp \left({\frac{\epsilon^2}{2\text{deg}_{\max} R^2}} \right)-1}\notag \\
& \leq  \sum_{S \in 2^V}  \sum_{ u \in S}　\frac{ 2 \exp \left( - \frac{k' \epsilon ^2}{2  \text{deg}_{\max} R^2} \right) }{ {\frac{\epsilon^2}{2\text{deg}_{\max} R^2}}}\notag \\
 & = \sum_{S \in 2^V}  \sum_{u \in S}  \frac{4 \text{deg}_{\max} R^2}{\epsilon^2} \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2 \tilde{ \log }(n-1)  } \right) \notag \\
%   & \leq \sum_{ S \in \tilde{{\cal S}} } \Pr \left[ \left| \text{deg}^*_{S}(v) - \widehat{\text{deg}}_{S}(v, T_t(v)) \right| \geq \epsilon    \right]. \\
%     & \leq  2(n-1) \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{8n^3  \text{deg}_{\max}R^2 \tilde{ \log }(n-1)   } \right),
&  \leq  \frac{4 \text{deg}_{\max}2^n n  R^2}{\epsilon^2} \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right),
\end{alignat}
where
%the first inequality follows by \eqref{ineq:prob_deg}, 
the third inequality follows by \eqref{ineq:hoeff_graph} and
the fourth inequality follows by $e^{-x} \geq 1-x$.
%and second inequality follows by \eqref{ineq:times}.
% Therefore, 
% using Hoeffding's inequality,
% we have 
% \begin{align}\label{ineq:hoeffding}
%     \Pr \left[  \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v) \right| \geq \epsilon \right] \leq 2 \exp \left( - \frac{\tilde{T}_t \epsilon^2 }{8n^2 |E_{S_{n-t+1}}(v)|R^2 } \right).
% % \end{align}

% By combining this inequality into \eqref{ineq:hoeffding},
% we have 
% \begin{align}
%       \Pr \left[  \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v) \right| \geq \epsilon \right] \leq 2 \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{8n^3 |E_{S_{n-t+1}}(v)|R^2 \tilde{ \log }(n-1)   } \right).  
% \end{align}

Now using ~\eqref{ineq:deg} and taking a union bound for all $t \in \{1, \ldots n-1 \}$ and all $v \in S_{n-t+1}$,
we obtain
\begin{alignat*}{4}
    \Pr   \left[  \bigcap_{t=1}^{n-1} \mathcal{E}_t' \right]= & 1- \Pr \left[ \exists t \in \{1, \ldots n-1 \}, v \in S_{n-t+1} \middle| \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v,t) \right| \geq \epsilon \right] \\
     & \geq  1- \sum_{t=1}^{n-1}\sum_{v \in S_{n-t+1}} \Pr \left[  \left| \text{deg}^*_{S_{n-t+1}}(v) - \widehat{\text{deg}}_{S_{n-t+1}}(v,t) \right| \geq \epsilon \right] \\
     & \geq 1  -   \sum_{t=1}^{n-1}\sum_{v \in S_{n-t+1}} \frac{4 \text{deg}_{\max}2^n n R^2 }{\epsilon^2}\exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right) \\
     %\geq 1  -   \sum_{t=1}^{n-1}  \frac{4 \text{deg}_{\max}R^2 n}{\epsilon^2} \exp \left(n- \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{16 n^2 (\text{deg}_{\max}+1)^2 R^2  \tilde{ \log }(n-1) } \right) \\
     & = 1  -  \frac{4 \text{deg}_{\max}2^n n R^2 }{\epsilon^2} \sum_{t=1}^{n-1}|S_{n-t+1}| \exp \left(- \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right) \\
     & = 1  -  \frac{4 \text{deg}_{\max}2^n n R^2 }{\epsilon^2} \sum_{t=1}^{n-1}(n-t+1) \exp \left(- \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right) \\
     & = 1- \frac{2 \text{deg}_{\max} 2^n R^2}{\epsilon^2} n^2(n+1) \exp \left(- \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max}R^2   \tilde{ \log }(n-1) } \right) \\
    & \geq 1- \frac{2 \text{deg}_{\max} 2^n R^2}{\epsilon^2}(n+1)^3 \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right).
\end{alignat*}

\end{proof}

\section{Proof of Theorem~\ref{thm:fixbudget}}


\begin{proof}
Now we are ready to prove Theorem~\ref{thm:fixbudget}.
First, we verify that the algorithms requires at most $T$ queries.
%In each phase $t$,  for a subset of vertices $S_{n-t+1}$,
%the algorithm calls the sampling oracle for  $\left \lceil  \tilde{T_t}-\tilde{T}_{t-1 \right  \rceil$ times.
%Thus, at the end of phase $n-1$, the algorithm uses at most $\frac{\tilde{T}_{n-1}}{2}+n-1$ queries.
In each phase $t$, the number of samples Algorithm~\ref{alg:sampling} requires is at most $\tilde{T_t}+ |S_{n-t+1}|$, since we have that 
\begin{align*}
\sum_{v \in S_{n-t+1}} \sum_{i=1}^t \tau_i 
=\sum_{v \in S_{n-t+1}} \sum_{i=1}^t T'_i - T'_{i-1} 
=\sum_{v \in S_{n-t+1}} T'_t 
\leq \sum_{v \in S_{n-t+1}}\left( \frac{\tilde{T}_t}{|S_{n-t+1}|}+1 \right)
\leq \tilde{T}_t+ |S_{n-t+1}|.
% &=\sum_{v \in S_{n-t+1}} (|N_{S_{n-t+1}}(v)|+1) \left\lceil  \frac{\tilde{T_t}}{ (|N_{S_{n-t+1}(v)}|+1)|S_{n-t+1}|} \right \rceil \\ 
% &\leq \sum_{v \in S_{n-t+1}} \left(   \frac{\tilde{T_t}}{ |S_{n-t+1}|}+|N_{S_{n-t+1}}(v)|+1 \right) \\ 
% & \leq \tilde{T_t} + (|S_{n-t+1}|+1)^2.
\end{align*}
%Therefore, Algorithm~\ref{alg:sampling} in total uses at most $\sum_{t=1}^{n-1}\tilde{T_t}-\tilde{T}_{t-1 =\frac{\tilde{T_{n-1}}}{2}$ samples.
% for $v \in S_{n-t+1}$,
% $T_t(v)$ is at most $\frac{\tilde{T}_t}{2}+t$ since we have
% \begin{align*}
% T_v(t) \leq \left(\sum_{i=1}^t \frac{\widetilde{T}_i - \widetilde{T}_{i-1}}{2 |S_{n-i+1}| |N_{S_{n-i+1}}(v)|}+1\right) \leq
% \left(\sum_{i=1}^t \frac{\widetilde{T}_i - \widetilde{T}_{i-1}}{2}\right)+t \leq \frac{\widetilde{T}_t}{2}+t.
% \end{align*}
% Therefore, we see that one subset of edges $E(S_n)$ is querie_ 
% for $\frac{\tilde{T}_1}{2} +1$ times, \ldots,
% and one subset of edges $E(S_1)$ for $ \frac{\tilde{T}_{n-1}}{2} +n-1$ times.
Therefore,
the total number of queries used by the algorithm is bounded by
\begin{alignat*}{4}
\sum_{t=1}^{n-1}\left( \tilde{T}_t+ |S_{n-t+1}| \right)
%& \leq \sum_{t=1}^{n-1} \left(\tilde{T_t}-\tilde{T}_{t-1}\right)+n-1 \\
& \leq  \sum_{t=1}^{n-1}\tilde{T_t}+\sum_{t=1}^{n-1}(n-t+1)   \\
& \leq \sum_{t=1}^{n-1} \left(  \frac{T-\sum_{i=1}^{n+1}i}{(n-t) \tilde{\log}(n-1) } +1 \right)+  \sum_{t=1}^{n-1}(n-t+1) \\
& \leq \sum_{t=1}^{n-1}  \frac{T-\sum_{i=1}^{n+1}i}{(n-t) \tilde{\log}(n-1) }+  \sum_{i=1}^{n+1}i \\
& = \frac{(T-\sum_{i=1}^{n+1}i)}{\tilde{\log}(n-1)} \tilde{\log}(n-1)  +\sum_{i=1}^{n+1}i \\
& = T- \sum_{i=1}^{n+1}i+\sum_{i=1}^{n+1}i=T.
\end{alignat*}

Lemma~\ref{lemma:fix_budget_lemma} implies that
the random event $\cE' := \bigcap_{t=1}^{n-1} \cE'_t$ occurs with probability at least $  1- \frac{2 \text{deg}_{\max} 2^n R^2}{\epsilon^2}(n+1)^3 \exp \left( - \frac{(T-\sum_{i=1}^{n+1}i) \epsilon^2 }{4 n^2 \text{deg}_{\max} R^2  \tilde{ \log }(n-1) } \right)$.
We shall assume the event $\cE'$ occurs in the rest of the proof,
because we only need to show that the algorithm outputs a solution $S_{\tt OUT}$ that guarantees $f_w(S_{\tt OUT}) \geq \frac{f_w(S^*)}{2} - \epsilon$ under $\cE'$.


%\subsection{Theoretical Guarantee of Peeling}
%We analyze the solution obtained by the peeling algorithm. 
Let $S^*\subseteq V$ be an optimal solution in terms of the expected weight $w$.
%Let us denote by $S_{\tt OUT} \subseteq V$ the output of the peeling algorithm for $G(V,E, \widehat{w}_t)$.
%The next theorem shows that if the true degrees and the estimated degrees of vertices are close, the solution of the peeling algorithm admits the theoretical guarantee. 
% %\begin{theorem}\label{thm:approx}
% Let $c$ be a real.
% Given $t>m$, if $|\text{deg}_S(v,w)-\text{deg}_S(v,\widehat{w}_t)|\leq c$ holds for any  $S\subseteq V$ and $v\in S$, it holds that 
% \begin{align*}
% d_w(S_{\tt OUT})\geq \frac{1}{2}d_w(S^*)-c.
% \end{align*}
% \end{theorem}
Choose an arbitrary vertex $v\in S^*$. 
From the optimality of $S^*\subseteq V$, it holds that
\begin{align*}
f_w(S^*)=\frac{w(S^*)}{|S^*|}\geq \frac{w(S^*\setminus \{v\})}{|S^*|-1}=f_w(S^*\setminus \{v\}). 
\end{align*}
By using the fact that $w(S^*\setminus \{v\}) = w(S^*) - \text{deg}^*_{S^*}(v)$, the above inequality can be transformed into 
\begin{align}\label{ineq:optimality}
\text{deg}^*_{S^*}(v)\geq f_w(S^*). 
\end{align}

Let $S_{\tau} \subseteq V$ be the last subset over the phases that satisfies $S_{\tau} \supseteq S^*$ and let $\tau \in [1, \ldots, n]$ be its phase.
Let $\tau_{\tt OUT}$ be the phase $t$ such that $S_{n-t+1}=S_{\tt OUT}$.
Then we have 
\begin{align*}
f_w(S_{\tt OUT})
&=\frac{\frac{1}{2}\sum_{v\in S_{\tt OUT}}\text{deg}^*_{S_{\tt OUT}}(v)}{|S_{\tt OUT}|}\notag\\
&\geq \frac{\frac{1}{2}\sum_{v\in S_{\tt OUT}} \left( \widehat{ \text{deg}}_{S_{\tt OUT}}(v,\tau_{\tt OUT}) -\epsilon \right)}{|S_{\tt OUT}|} \notag\\
&\geq \frac{\frac{1}{2}\sum_{v\in S_\tau}
\widehat{ \text{deg}}_{S_{\tau}}(v, \tau)}{|S_{\tau}|}-\frac{\epsilon}{2}.
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tau}}\text{deg}_{S_{\tau}}(v)}{|S_{\tau}|}-\epsilon\\
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tau}}\text{deg}_{S^*}(v)}{|S_{\tau}|}-\epsilon \geq \frac{1}{2} f_w(S^*)-\epsilon, 
  \end{align*}
where
the first inequality follows from event $\cE'$,
the second inequality follows from the greedy choice of $S_{\tt OUT}$.
Recall that  the algorithm removes the vertex that satisfies $v_\tau \in \argmin_{v \in S_{\tau}} \widehat{ \text{deg}}_{S_{\tau}}(v, \tau)$ in the phase $\tau$.
Therefore, from the definition of $S_\tau$, it is clear that $v_\tau \in S^*$.
Using this property, we further have that
\begin{align*}
\frac{\frac{1}{2}\sum_{v\in S_{\tau}}
\widehat{ \text{deg}}_{S_{\tau}}(v, \tau)}{|S_{\tau}|}-\frac{\epsilon}{2}
& \geq \frac{\frac{1}{2}\sum_{v \in S_{\tau}}
\widehat{ \text{deg}}_{S_{\tau}}(v_\tau, \tau)}{|S_{\tau}|}-\frac{\epsilon}{2} \\
&=\frac{1}{2}
\widehat{ \text{deg}}_{S_{\tau}}(v_\tau, \tau)-\frac{\epsilon}{2} \\
& \geq \frac{1}{2}
 \text{deg}^*_{S_{\tau}}(v_\tau)-\epsilon \\
 & \geq \frac{1}{2}
 \text{deg}^*_{S^*}(v_\tau)-\epsilon \\
  & \geq \frac{1}{2}
 f_w(S^*)-\epsilon,
%\frac{\frac{1}{2}\sum_{v\in S_{\tt OUT}}\text{deg}^*_{S_{\tt OUT}}(v)}{|S_{\tt OUT}|}\\
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tt OUT}}\widehat{ \text{deg}}_{S_{\tt OUT}}(v)}{|S_{\tt OUT}|}-\frac{\epsilon}{2}\\
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tau}}
% \widehat{ \text{deg}}_{S_{\tau}}(v)}{|S_{\tau}|}-\frac{\epsilon}{2}.
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tau}}\text{deg}_{S_{\tau}}(v)}{|S_{\tau}|}-\epsilon\\
% &\geq \frac{\frac{1}{2}\sum_{v\in S_{\tau}}\text{deg}_{S^*}(v)}{|S_{\tau}|}-\epsilon \geq \frac{1}{2} f_w(S^*)-\epsilon, 
\end{align*}
where the second inequality follows from event $\cE'$, and third inequality follows  from the fact $S_{\tau}\supseteq S^*$, 
and the last inequality follows from the fact $v_{\tau} \in S^*$ and inequality (\ref{ineq:optimality}). 
Therefore, we obtain $f_w(S_{\tt OUT}) \geq \frac{1}{2}
 f_w(S^*)-\epsilon$. That concludes the proof.

\end{proof}

\clearpage


\begin{figure*}[t!]
\begin{center}
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/karate_sol.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/lemis_sol.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/polbooks_sol.pdf}
  }\\
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/adjnoun_sol.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/Jazz_sol.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/Email_sol.pdf}
  }
  \caption{Results for the behavior of our proposed algorithm with respect to the number of iterations. Each point is an average over 10 runs of the algorithm.}\label{fig:solution}
  \end{center}
\end{figure*}



\begin{figure*}[t!]
\begin{center}
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/karate_norm.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/lemis_norm.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/polbooks_norm.pdf}
  }\\
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/adjnoun_norm.pdf}
  }
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/Jazz_norm.pdf}
  }2
 \subfigure{
   \includegraphics[width=0.27\textwidth]{fig/Email_norm.pdf}
  }
  \caption{Results for the estimation of the expected weight $w$. Each point is an average over 10 runs of the algorithm.}\label{fig:norm}
  \end{center}
\end{figure*}




\section{Details of Experiments for \textsf{DS-Lin}}~\label{apx:exp}
\subsection{Behavior of \textsf{DS-Lin}}

We analyze the behavior of our proposed algorithm with respect to the number of iterations. 
In the previous section, we confirmed that the solution obtained after 10,000 iterations is almost densest in terms of unknown $w$. 
A natural question here is how the density of solutions approaches to such a sufficiently large value. 
In other words, does our algorithm is sensitive to the choice of the number of iterations? 
In this section, we answer these questions by conducting the following experiments. 
We terminate the while-loop of our algorithm once the number of iterations exceeds $0, 100, 200, \dots$, 10,000, 
and follow the density values of solutions in terms of $w$. 
For each instance, we again run our algorithm for ten times, and report the average value. 

The results are shown in Figure~\ref{fig:solution}. 
As can be seen, as the number of iterations increases, the density value converges to the sufficiently large value (close to the optimum). 
Although the density value sometimes drops down, the decrease is quite small. 
%Note that the algorithm outputs $S\subseteq V$ with a relatively large density even in an early stage,
%which implies that the algorithm reasonably estimates the true edge weight $w$ in a few iterations after the initialization step. 
%From the above, it can deduced that our algorithm is not sensitive to the choice of the number of iterations. 
%iteraetionが少ないと大きいデータでは動かないし，これは言い過ぎかと思いました．



\subsection{Estimation of the expected weight}
We explain the reason why our proposed algorithm \textsf{DS-Lin} performs fairly well. 
%Finally, we explain the reason why our proposed algorithm performs well. 
To this end, we focus on the quality of the estimated edge weight obtained by the algorithm. 
We measure the quality of the estimated edge weight $\widehat{w}_t$ by comparing with the expected weight $w$; 
specifically, we compute $\|w -\widehat{w}_t\|_1/m$. 
The experimental setup is exactly the same as that in the previous section. 

The results are depicted in Figure~\ref{fig:norm}. 
As can be seen, as the number of iterations increases, $\widehat{w}_t$ converges to the true edge weight $w$. 
It is very likely that the high performance of our algorithm is derived from the high-quality estimation of the expected edge weight $w$. 


\begin{algorithm}[t]\label{alg:roracle}
\caption{Robust optimization with oracle intervals (\textsf{R-Oracle})}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{ Graph $G=(V,E)$, oracle intervals $W=\times_{e \in E}[l_e, r_e]$ where $l_e=\min\{w_e-1,0 \}$ and $r_e=w_e+1$, sampling oracle, $\gamma \in (0,1)$, and $\varepsilon>0$}
	\Output{($S_{\rm out})$ }
	
    \For{each $e \in E$}{

    \If{$l_e=r_e$ }{
    $l^{\rm out}_e \leftarrow l_e, r^{\rm out}_e \leftarrow r_e$;
    }
    \Else{
    $S^*_{w^{-}} \leftarrow $ Output of Charikar's LP-based exact algorithm for $G(V,E, w^{-})$;
    
   $t_e \leftarrow \left\lceil  \frac{m(r_e-l_e)^2 \ln{\frac{2m}{\gamma}} }{ \varepsilon^2 f_{w^{-}}(S^*_{w^{-}})^2   } \right\rceil $;
  

    Sample $e$ for $t_e$ times;
    
    $\hat{p}_e \leftarrow \hat{X}_e(t_e)$;
    
    $\delta \leftarrow \frac{\varepsilon f_{w^{-}}(S^*_{w^{-}})}{\sqrt{2m}} $;
    
    $l_e^{\rm out} \leftarrow \max \{ l_e, \hat{p}_e-\delta \}$ and $ r^{\rm out}_e \leftarrow \min \{ r_e, \hat{p}_e +\delta \}$;
    }
    }
    
    
    $W_{\rm out} \leftarrow \times_{e \in E}[l^{\rm out}_e, r^{\rm out}_e]$;


    $S_{\rm out} \leftarrow$ Output of Charikar's LP-based exact algorithm for $G(V,E, l^{-}_{\rm out})$;
        
    \Return{
    $S_{\rm out}$;
    }
\end{algorithm}


\section{ Details of Experiments for \textsf{DS-SR}}\label{apx:dssr}






\begin{figure*}[t!]
\begin{center}
\subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/karate.pdf}
  }
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/lemis.pdf}
  }\\
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/polbooks.pdf}
  }
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/adjnoun.pdf}
  }\\
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/jazz.pdf}
  }
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/email.pdf}
  }\\
  \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/polblogs.pdf}
  }
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/email-Eu-core.pdf}
  }\\
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/facebook_combined.pdf}
  }
 \subfigure{
  \includegraphics[width=0.31\textwidth]{fig/sample/Wiki-Vote.pdf}
  }
  
  \caption{Fraction of the size of queried edge subsets in \textsf{DS-SR} (cumulative) over 100 generalizations.}\label{fig:cumlative_all}
  \end{center}
\end{figure*}

\subsection{Description of \textsf{R-Oracle} }
We describe the entire procedure of \textsf{R-Oracle} in Algorithm~\ref{alg:roracle}.
This algorithm employs the robust optimization model proposed by~\citet{Miyauchi_Takeda_18}.
Their robust optimization model takes intervals of edge weights as its input.
We generate the intervals $W= \times_{e \in E}[l_e, r_e]$ based on unknown edge weight $w$, i.e., $l_e=\min\{w_e-1,0 \}$ and $r_e=w_e+1$. 
Algorithm~\ref{alg:roracle} first obtains the optimal solution $S^*_{w^{-}}$ in terms of extreme edge weight $w^{-}=(l_e)_{e \in E}$ and computes the value of $f_{w^{-}}(S^*_{w^{-}})$.
Then, for each single edge $e \in E$,
the algorithm calls the sampling oracle for an appropriate number of times and obtains the empirical mean. Using the empirical means, the algorithm constructs intervals $W_{\rm out} \leftarrow \times_{e \in E}[l^{\rm out}_e, r^{\rm out}_e]$,
and computes a densest subgraph $S_{\rm out}$ on $G$ with $w^{-}_{\rm out}=(l^{\rm out}_e)_{e \in E}$.

\subsection{ The number of samples for single edges in \textsf{DS-SR}}
We report experimental results on the size of queried edge subsets in \textsf{DS-SR} (cumulative) over 100 generalizations for all instances in Figure~\ref{fig:cumlative_all}.



\end{onecolumn}
